ScriptViz: A Visualization Tool to Aid Scriptwriting based on a Large Movie Database

Scriptwriters usually rely on their mental visualization to create a vivid story by using their imagination to see, feel, and experience the scenes they are writing. Besides mental visualization, they often refer to existing images or scenes in movies and analyze the visual elements to create a certain mood or atmosphere. In this paper, we develop ScriptViz to provide external visualization based on a large movie database for the screenwriting process. It retrieves reference visuals on the fly based on scripts' text and dialogue from a large movie database. The tool provides two types of control on visual elements that enable writers to 1) see exactly what they want with fixed visual elements and 2) see variances in uncertain elements. User evaluation among 15 scriptwriters shows that ScriptViz is able to present scriptwriters with consistent yet diverse visual possibilities, aligning closely with their scripts and helping their creation.

==> alt-text.tex <==
Figure 1. A scriptwriter writes a main character “Dave", who is irritable and impulsive, trapped in a desert. She has a few sentences in her mind as shown in the top. She wants to choose an appropriate setting on time-of-day and the other character’s gender at the beginning of her creation. By setting these as variant attributes, she sees different visualizations in three rows and prefers the 3rd one. The night view she sees better reflects characters’ bad situations as they are tired for a whole day. The dead tree in the background strengthens this tension and also changes her script by adding details into it (bolded red text) at the bottom. These additions create a better main character by enhancing Dave’s personality. After seeing the visualization, it helps to add details that better reflect characters’ desperate situation. The interface is shown in the supplementary video.

Figure 2: The pipeline of ScriptViz. It first preprocesses the database and retrieves scenes according to user’s input. It is based on two types of control on visual attributes that enable writers to 1) see exactly what they want with fixed visual elements and 2) see variances in uncertain elements. It then retrieves images for each script’s dialogue sequences.

Figure 3: Preprocess database. Setting: we compute the CLIP [Radford et al . 2021] visual-text similarity between setting tags and visual frames to acquire recognizability score of setting tags for each frame. Cast: we detect the front face to acquire a recognizability score for each character in each frame.

Figure 4: A screenwriter types in a script and selects their story’s fixed and variable attributes. ScriptViz retrieves sequences for the input script. The screenwriter iterates on the script based on the proposed sequences. After seeing the visualization, it helps to enrich the details of the existing dialogue and write the unfinished dialogue.

Figure 5: Comparison of visualization via changing the location attributes from "Restaurant" to "Dining Room" in the SQL input.

Figure 6: Comparison of visualization via changing the location attributes from "Living Room" to "Car" in the SQL input.

Figure 7: Questionnaire results.

Figure 8: Qualitative clarity comparison of different approaches.

Figure 9: The visualization results in the location value outside the category list in MovieNet via computing the text-visual similarity between the textual CLIP embedding of user input and the visual CLIP embedding extracted from the establishing shot’s keyframe of each scene. Noting that the “desert" in the teaser image does not belong to the existing category list, we show more results here, such as “Snowy Forest," “Ice Cave," and “Canyon in Desert."

Table 1: Information about the participants of the system
evaluation.

Table 2: Time comparison of using different approaches to
write scripts that reach writers’ expectations.

Table 3: Quantitative clarity comparison of different approaches.


